A Malaria Control Model Using Mobility Data: An Early Explanation of Kedougou's Case in Senegal

Studies in malaria control cover many areas such as medicine, sociology, biology, mathematic, physic, computer science and so forth. Researches in the realm of mathematic are conducted to predict the occurrence of the disease and to support the eradication process. Basically, the modeling methodology is predominantly deterministic and differential equation based while selecting clinical and biological features that seem to be important. Yet, if the individual characteristics matter when modeling the disease, the overall estimation of the malaria is not done based on the health status of each individual but in a non-specified percentage of the global population. The goal of this paper is to propose a model that relies on a daily evolution of the individual's state, which depends on their mobility and the characteristics of the area they visit. Thus, the mobility data of a single person moving from one area to another, gathered thanks to mobile networks, is the essential building block to predict the outcome of the disease. We implement our solution and demonstrate its effectiveness through empirical experiments. The results show how promising the model is in providing possible insights into the failure of the disease control in the Kedougou region.

==> sections/Annexes.tex <==
\section{Appendix}
\label{annexe}
\subsection*{Patches Parameters}
\label{annex1}
In Table \ref{table2}, we give the parameters related to each patch. 
%We recall that computing the value of parameters listed in Table \ref{table2} required additional informations that we ignore in this paper for  sake of conciseness. 
We refer the reader to the work presented in \cite{Chitnis2008,Gao2012} for more parameter details. 
\begin{table}[h]
\rowcolors{2}{lightgray}{white}
\caption{Patches Parameters}
\renewcommand{\arraystretch}{0.8}% Tighter
\begin{tabular}{|c|p{9.5cm}|}
\hline
\textbf{Parameter} & \textbf{Description} \\
\hline
$N_h^i(t)$ & Human population in patch $i$ at time $t$\\
\hline
$N_v^i(t)$ & Vector Population in patch $i$ at time $t$\\
\hline
$I_v^i(t)$ & Infected mosquitoes in patch $i$ at time $t$\\
\hline
$I_h^i(t)$ & Infected humans in patch $i$ at time $t$\\
\hline
$R_h^i(t)$ & Infected individuals in patch $i$ that recover at time $t$\\
\hline
$\beta^i_{HV}$  & Probability that an infectious person infects a susceptible mosquito during a contact within the patch $i$\\
\hline
$\beta^i_{VH}$ & Probability that an infectious mosquito infects a susceptible individual during a bite in patch $i$\\
\hline
$\tilde{\beta}^i_{HV}$ &Probability that a recovered person infects a susceptible mosquito during a contact in patch $i$\\
\hline
$b^i_h(t)$  & Proportion of bites per human per unit time $t$ in patch $i$\\
\hline
$b^i_v(t)$  & Proportion of bites per mosquito per unit time $t$ in patch $i$\\
\hline
$\lambda^i_{VH}$  & Force of infection from vector to human  in patch $i$, \textit{i.e.,} measure of how likely a human get exposed in patch $i$\\
\hline
$\lambda^i_{HV}$  & Force of infection from human to vector  in patch $i$, \textit{i.e.,} measure of how likely a mosquito get exposed in patch $i$\\ 
%}
\hline
\end{tabular}
\label{table2}
\end{table}

\subsection*{Individual Parameters}

We may rely on the literature to set the parameter values described in Table \ref{table3}  to assess whether an individual switches over the different SEIR classes. For instance, $h_j$ is likely to move to $I$ class after a period of $ \frac{1}{\nu_{h, j}}$ and, later on, to $R$ class after a period of $ \frac{1}{\gamma_{h, j}}$.
\label{annex2}
\begin{table}[h]
\rowcolors{2}{lightgray}{white}
\caption{Individual Parameters for a given time window}
\begin{tabular}{|c|p{10cm}|}
\hline
\textbf{Parameter} & \textbf{Description} \\
\hline
$h_j$ & Identification of the individual $j$ \\
\hline
%$d_j^{k}$ & Time interval that  $h_j$ spends visiting patch $k$ during the time window $W$; \\
%\hline
$w_j^{k}$  & Visiting ratio of time that $h_j$ spends in patch $k$.
%; $w_j^{k} = \frac{d_j^{k}}{W}$ 
\\
\hline
$S_{h,j}(t)$ & Susceptible state variable of $ h_j $ at time step $ t $ (1 if susceptible 0 otherwise)\\
\hline
$E_{h,j}(t)$ & Exposed state variable of $ h_j $ at time step $ t $ (1 if exposed 0 otherwise)\\
\hline
$I_{h,j}(t)$ & Infected state variable of $ h_j $ at time step $ t $ (1 if infected 0 otherwise)\\
\hline
$R_{h,j}(t)$ & Recovered state variable of $ h_j $ at time step $ t $ (1 if recovered 0 otherwise)\\
\hline
$pe_j(t)$ & Probability that individual $h_j$ (being in class $S$) moves to class $E$
%residing in patch $i$ 
%moves from $S$ class to the $E$ one
% \\
% \hline
% $pi_j(t)$ & Probability that $h_j$ in class E moves to class $I$
% %residing in patch $i$ 
% %moves from $E$ class to the $I$ one
% \\
% \hline
% $pr_j(t)$ & Probability that $h_j$ in class I moves to class $R$
% %residing in patch $i$ 
% %moves from $I$ class to the $R$ one
% \\
% \hline
% $ps_j(t)$ & Probability that $h_j$ goes back to class $S$
% %residing in patch $i$ 
%moves from $S$ class to the $E$ one
\\
\hline
$\nu_{h,j}$ &  
% Latency rate ($day^{-1}$) of individual $j$. 
 incubation period (without symptoms). In the case of P. falciparum parasite, which predominates in Senegal, it varies from 9 to 10 days \cite{Chitnis2008,Cdc2015}.\\
\hline
$ \frac{1}{\gamma_{h, j}}$ & 
% Infectivity rate ($ day^{- 1} $) of the individual $j$. 
is the infectious period (Chitnis and Al. have set it at 9.5 months \cite{Chitnis2008})\\
% Without treatment, it varies between 12 and 24 months \cite{Williams2002}. 
% In their model Chitnis and Al. have set it at 9.5 months \cite{Chitnis2008}.\\
% \hline
% $ \rho_{h,j} $ & Loss of immunity rate ($ day^{- 1} $) of the individual $ j $. $ \frac{1}{\rho_{h, j}} $ is the duration of the immunity period. Chitnis et al. set it at 1 year for low transmission zones and 5 years for high transmission zones \cite{Chitnis2008}. \idy {on ne l'utilise pas dans le reste }\\
\hline

%$ s_j $ & Immunity threshold beyond which the individual $j$ becomes exposed. \\
\hline

\end{tabular}
\label{table3}
\end{table}

 \subsection*{Individual-based Malaria Model Transmission}
 \label{annex3}
With the previous parameters, we may define the flowchart of the disease by gathering individual transitions.
In this respect, we add the number of individuals belonging to each class for each patch in a regular basis (each night for example). Thus, individuals of a class are known as precisely located in a patch.   
The variation of the human population over the different classes are formalized as follows :

\begin{equation*}
  %  2 EQUATIONS PAR LIGNE
 \begin{split}
 	& S^i_h(t)= \sum\limits_{j=1}^M w^i_j(t)~ S_{h,j}(t) \hspace{1cm} E^i_h(t)= \sum\limits_{j=1}^M w^i_j(t)~ E_{h,j}(t) \\
%    & E^i_h(t)= \sum\limits_{j=1}^M w^i_j(t)~ E_{h,j}(t) \\
    & I^i_h(t)= \sum\limits_{j=1}^M w^i_j(t)~ I_{h,j}(t) \hspace{1cm} R^i_h(t)= \sum\limits_{j=1}^M w^i_j(t)~ R_{h,j}(t)\\
%    & R^i_h(t)= \sum\limits_{j=1}^M w^i_j(t)~ R_{h,j}(t)\\
 \end{split}
\end{equation*}
   
The variation of mosquitoes population over the classes, are exactly the same described in \cite{Chitnis2008} and obtain the following :  
  \begin{equation*}
 \begin{split}
  	& \frac{dS^i_v}{dt}= \psi^i_v N^i_v - \lambda^i_{HV}(t) S^i_v - f^i_v(N^i_v) S^i_v \hspace{1cm} \frac{dI^i_v}{dt}=\nu^i_v E^i_v - f^i_v(N^i_v) I^i_v\\
    & \frac{dE^i_v}{dt}= \lambda^i_{HV}(t) S^i_v - \nu^i_v E^i_v - f^i_v(N^i_v) E^i_v \\
%    & \frac{dI^i_v}{dt}=\nu^i_v E^i_v - f^i_v(N^i_v) I^i_v\\
 \end{split}
\end{equation*}
where $f^i_v(N^i_v) = \mu_{1v}^{i} + \mu_{2v}^{i} N^i_v$  is the per capita density-dependent death rate for mosquitoes in the patch $i$ \cite{Chitnis2006}.

 It is worth noting that after each time unit, we update data related to the patches and the individuals such as the FoI and the health status since they are used as input for the next time step.
 



==> sections/conclu.tex <==
\section{Conclusion}
In this article we proposed a malaria model that takes into account user informations such as their mobility pattern, their health status, and so on.
The model is a discrete SEIR-SIS approach and differs mainly to existing models by the fact that global details of the disease are obtained by gathering the health status of each individual of a given population. Our approach is more accurate in terms of estimating the disease scoop and afford the possibility to build a more efficient vector control for eliminating malaria in Africa. Actually, our model is an early explanation of Kedougou's case where the malaria incidence is still high despite the strategies of the Senegal national program. In this respect, it unveils kind of solutions that decision makers  can use with respect to individuals movement in order to eliminate the disease.
Moreover, the results from our model match real observations in Kedougou with a mean absolute error of 0.001 while using synthetic data. Such a result is  promising and let us believe that with real data, our approach will behave efficiently. Thus, ongoing works are conducted to collect  on-line mobility data obtained, for instance, through mobile networks.  
{\bf We are aware that the results presented in this paper are mainly based on synthetic data and thus cannot be interpreted as realistic results. However, as we obtain expected values (corresponding to a natural intuition), we believe that our model behaves correctly and should give useful information when applied to real data in the future}


==> sections/problem.tex <==
\section{Motivating Example}
\label{sec:pb}

\color{blue}
We want to optimize malaria vector control by detecting on real-time in which (fine grain) regions the disease is likely to appear/spread. We show in this section that taking the mobility of individuals into account greatly helps in understanding the situation and take the appropriate control action.

% \subsection{Motivating example}


% \paragraph{Basic example showing the impact of people mobility on the overall number of exposed persons}
% We sketch an example to illustrate the effect of 
% people moving across areas.
% %
% Let's start with a single area $A$ with a known infection strength, hosting 100 people including one infected person. Applying the model on $A$. We get 10 people exposed after one month, and a total of 40 people exposed after the next month.
% Notice that the infection strength has increased from month 1 to month 2 because more vectors have been infected as defined by the Malaria model (the actual values of the infection strength are not needed to understand the example).

% We now compare this simple case with a case where people can move. We split $A$ into areas $A_1$ and $A_2$ having the same infection strength as $A$, and hosting 50 people each. Initially, the only infected person lives in $A_1$, and $A_2$ host only healthy people.
% We still consider a period of 2 months and detail the people moves that occur at the beginning of each month.
% At the beginning of the first month, the 50 people from $A_1$ move to $A_2$. Applying the model, we get 10 people exposed in $A_2$ after one month. As a consequence the infection strength of $A_2$ has increased whereas in $A_1$ the infection strength remained at its initial value. Then at the beginning of the second month, suppose that everyone move to $A_1$ and stay there. We end up with a total of $20$ people infected.  This is twice less than what we got in the no-moving case.

% Through this example, we see that people gathering to a specific area tend to boost the infection strength of that area. We also see that the infection strength 'sticks' within an area: when people are moving it does not effect in 'transmitting' the infection strength between areas. This is because the transmission vectors (mosquitoes) do not move outside an area. This assumption is realistic even for 'small' area of a few km2.


We sketch an example about the evolution of malaria when people are moving.
We compare two approaches that describe people movement either at a coarse grain or at a finer grain.
(i) The coarse-grained \textbf{global} approach considers global migration ratio from a patch to another patch. % a  (at a larger spatial scale).
(ii) The fine-grained \textbf{personalized} approach considers geo-position info (\ie GPS coordinates) about identified users. %with high precision less than a few meters
The Figure~\ref{exple:persmove} illustrates that the personalized approach captures the 
mobility % malaria dynamics 
more accurately than the global one.
It shows 3 persons living in a residential patch. Every day some of the persons visit an \textit{ad-hoc} patch (meeting point) and come back home.

\begin{figure}[hptb]
\includegraphics[width=1\linewidth]{images/exple1d.png}
\caption{Global mobility vs. Personalized mobility}
\label{exple:persmove}
\end{figure}
\vspace{-0.5cm}

In the case (i) (see Figure~\ref{exple:persmove}(a)), 
the mobility is  defined as a ratio : every day 33\% of the individuals (\ie one person out of 3) is randomly selected to move to an ad-hoc patch. 
Therefore, eventually everyone spends the same amount of time out of its residential patch. The mobility pattern is homogeneous and global to the group of people living in the residential patch.

In the personalized case, Figure~\ref{exple:persmove}(b), 
the mobile individuals are identified. $H_1$ is the only mobile person. Although the average mobility in (b) is the same as in (a), $H_1$ is 3 times more mobile than the persons of scenario (a).

Suppose that the risk for someone to become exposed is proportional to the time spent in an infected patch.
Let us say that someone become exposed after 10 visits.
We compare the global vs. personalized mobility scenario when the visited \textit{ad-hoc} patch is infected. % which tend to make a visitor exposed. 
In the case of global mobility many users will become exposed slowly (3 people exposed at day 30), whereas in the case of personalized mobility fewer users will become exposed faster ($H_1$ is exposed at day 10).

Suppose now a decision maker who expects to be alerted when the amount of exposed people reaches 10\%. The personalized mobility scenario succeeds to trigger the alert at day 10.
In the global mobility scenario, the alert is triggered at day 30, which could be too late to prevent the epidemic propagation.

That example illustrates the importance to take into account personalized mobility in the modeling of the malaria propagation.

\color{black}


% -------------------------------------------------------------
% Example à partir de vraies données sur le nombre d'infectés
% -------------------------------------------------------------
% Let's continue the above example, and detail the evolution of the desease at each area, expressed as a percentage of new infected people by month 
% (\cf Fig XX %Fig~\ref{fig:is} 
% for a sample of real values over months in several districts of Dakar).
% \hub{Est-ce qu'on ajoute ici le tableau donnant les nb d'infectés réels mesurés à Dakar ?}
% \idy{On est confronté à un problème d'espace}



% -------------------------------------
%          Exemple avec 3 zones
% -------------------------------------
% In $A_1$ we have $IS_{A_1}=10\%$, in $A_2$ we have $IS_2=30\%$.
% Suppose another area $B$ hosting 100+ people.
% If 100 people from $B$ migrate to $A_1$, we get 10 exposed persons after one month as well as an increase for $IS_{A_1}=12\%$. If those 100 people would have migrated to $A_2$ (instead of $A_1$), we would have got 30 exposed persons after one month, and $IS_{A_2}=50\%$.

% Consider now the more global case where we do not know whether people are migrating to $A_1$ or $A_2$. We only know that 100 people from $B$ migrate to $A$ which has an average value $IS_A=20\%$. Thus we get 20 exposed people which may deviate from the actual number of exposed people (10 or 30), and $IS_A=25\%$.


% \hub{
% %Suite à la discussion du vendredi 7/7, un autre exemple plus adéquat serait celui-ci:
% ENLEVER/fusionner LA SUITE ?
% }

% \paragraph{Example showing that individual (\ie personalized) information about who is healthy, exposed, or infected, allows to better predict what will be the $FoI$ of an area on the forthcoming days}.
 
% %healthy vs infected person moving

% Case 1: an healthy person moves from A to B (one night) then come back to A and stay there. As few days later the $IS$ of B is still at its initial value

% Case 2: an infected person moves from A to B (one night) then come back to A and stay there. As few days later the IS of B is higher than in case 1.



% [19/7]: 
%Case 3: cas visant à illustrer l'avantage dans le modèle personnalisé de connaitre les déplacements successifs d'une certaine personne, jour après jour. 
%Cette info (si j'ai bien compris l'état de l'art) n'est pas connue dans les solutions existantes: ce qui est connu est seulement qu'une portion des personnes de A est allée en B, puis le lendemain une autre portion de A est allée en C, mais on ne sait pas si ce sont les même personnes qui ont effectué les 2 déplacements A vers B puis de A vers C. 





% -------------------------------------
% CHALLENGES
% -------------------------------------
% \subsection{Challenges}
%\subsection{Position wrt. related works and Challenges}
% \label{defi}



% We face the following challenges:
% Leverage on personalized and real time mobility information to know more precisely the evolution of the malaria in the large area composed of 
%estimate the health state of each person. 
%  Improve 


% \hub{
% Insister sur les uses-case qu'on cible avec notre modele et le benefice attendu.

% Use case 1: suivi individualisé de l'état de santé d'une personne
% (corespond à l'exéprience 1)

% Use case 2: suivi de l'état d'une zone (expérience 2)

% Use case 3: planification de la démoustiquation : où et quand démoustiquer
% }

% The first challenge is to integrate user mobility information to improve the 'accuracy' of a malaria prediction model.
 
% The second challenge is to design an 'expressive' malaria prediction model. The model should be able to describe users that have dynamic mobility patterns that may evolve depending on the user state. Notably, the model has to describe a mobility pattern that depends on the state (S,E,I,R) of the user.
 
 
 
 
% ------------------------------------------------------------
%               RELATED WORKS
% ------------------------------------------------------------
 
 
%\subsection{Position wrt. existing solutions}

% HN: A DEPLACER 
%Since the seminal work of Ross~\cite{Ross1911} which defined the first compartmental model called SIR,
% %(for Susceptible - Infectious - Recovered)
% there have been a century of research that lead to many extended models~\cite{Filipe2007} with more compartments (\eg Exposed), more transitions (\eg bridging the Human and Vector models), and aware of various parameters (\eg vector density, immunity) and contextual information (\eg human migration, spatial position) to achieve better accuracy and usability. 

% In our context of real time monitoring of malaria propagation based on mobility information, we rely on ~\cite{Chitnis2006} because it provides accurate bites estimation and  takes into account latency, infectivity and immunity
% However, \cite{Chitnis2006} has 2 limitations : the lack of spatial diversity (the model considers only a single area with homogeneous parameters) and consequently the lack of mobility: people remain in the area. 




% One of the first model, known as the classical "Ross model", is developed by Sir Ronald Ross, which explained the relationship between the number of mosquitoes and incidence of malaria in humans~\cite{Ross1911}. The model was devised by considering three health status (compartments) that states for SIR – S for the susceptible to the infection, I for the infectious, and R for the recovered (or immune). The variables S, I, and R represent the number of people in each compartment at a particular time. 
% The model is deliberately a simplified set of concepts that serves as a basis for building countless other models of mosquito-borne disease transmission~\cite{Filipe2007}.


% \begin{table}[]
% \centering
% \caption{Comparison of models}
% \label{t:comparisonModels}
% \resizebox{\textwidth}{!}{\begin{tabular}{ccccccc}
% \hline
% \rowcolor[HTML]{gray} 
% \textbf{Model} & \textbf{Vector bites~}          & \textbf{Latency~}           & \textbf{Infectivity~}       & \textbf{Immunity~}          & \textbf{heterogeneity}                            & \textbf{Mobility}                                           \\ \hline
% 2006 ~\cite{Chitnis2006}          & {\color[HTML]{009901} accurate}   & {\color[HTML]{009901} yes} & {\color[HTML]{009901} yes} & {\color[HTML]{009901} yes} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{CB0000} no} & {\color[HTML]{CB0000} immigration of susceptibles} \\
% 2012 ~\cite{Gao2012}          & {\color[HTML]{CB0000} inaccurate} & {\color[HTML]{009901} yes} & {\color[HTML]{009901} yes} & {\color[HTML]{009901} yes} & {\color[HTML]{009901} yes}                        & {\color[HTML]{F56B00} travel rates}                         \\
% 2016 \cite{Ruktanonchai2016}          & {\color[HTML]{FE0000} inaccurate} & {\color[HTML]{CB0000} no}  & {\color[HTML]{009901} yes} & {\color[HTML]{CB0000} no}  & {\color[HTML]{009901} yes}                        & {\color[HTML]{FFC702} not in real time}                     \\
% Proposed model & {\color[HTML]{009901} accurate}   & {\color[HTML]{009901} yes} & {\color[HTML]{009901} yes} & {\color[HTML]{009901} yes} & {\color[HTML]{009901} yes}                        & {\color[HTML]{009901} in real time}                         \\ \hline
% \end{tabular}}
% \end{table}



% \lynda{A réécrire : The table \ref{t:comparisonModels}, summarizes some of the work done in malaria modeling. The Chitnis \cite{Chitnis2006} model provides an accuracy in calculating the number of vector bites. Indeed, they modify the calculation of their predecessors Ngwa and Shu \cite{NGWA2000}, which rely only on the density of the vectors, and take into account the relative density of humans and vectors in the area. Moreover, their model takes into account the latency periods of humans and vectors, and the human immunity period. However, it assumes that the whole area is homogeneous and take into account, only, a constant immigration of a susceptible human population. In 2012, Gao and Ruan \cite{Gao2012} use the multi-patch concept to introduce heterogeneity of areas and use travel rates between patches to simulate displacements. However, their model based on that of Ngwa and Shu \cite{NGWA2000}, lacks accuracy in calculating the number of bites per night per area. In addition, they do not take real travel into account. In 2016, Ruktanonchai \cite{Ruktanonchai2016} considers real mobility data for a part of the population in Namibia over a specified period of time. However, they use an overly simple model that does not take into account the latency and immunity periods. We want to design the most realistic model based on that of Chitnis. We introduce the heterogeneity of the zones thanks to the multipatch concept and bring more precision in terms of displacement by making our model able to take into account real-time mobility data.}
% %pooints évoqués le 7/7
% \paragraph{comparaison avec PLOS2016}

% - SIR   \textcolor{cyan}{D'après l'équation, je crois même que c'est SIS (les infectieux redeviennent sains)} et pas SEIR

% - pas personalisé

% - trop homogène car trop agrégé

% -pas en temps réel, basé sur des données historiques concernant une période ancienne (au moins 5 ans d'age, rien sur les 5 dernières années)





 
% \subsection{Overview of proposed methods}
% [TODO]










